DeCoAR 2.0: Deep Contextualized Acoustic Representations with Vector Quantization

Recent success in speech representation learning enables a new way to leverage unlabeled data to train speech recognition model. In speech representation learning, a large amount of unlabeled data is used in a self-supervised manner to learn a feature representation. Then a smaller amount of labeled data is used to train a downstream ASR system using the new feature representations. Based on our previous work DeCoAR and inspirations from other speech representation learning, we propose DeCoAR 2.0, a Deep Contextualized Acoustic Representation with vector quantization. We introduce several modifications over the DeCoAR: first, we use Transformers in encoding module instead of LSTMs; second, we introduce a vector quantization layer between encoder and reconstruction modules; third, we propose an objective that combines the reconstructive loss with vector quantization diversity loss to train speech representations. Our experiments show consistent improvements over other speech representations in different data-sparse scenarios. Without fine-tuning, a light-weight ASR model trained on 10 hours of LibriSpeech labeled data with DeCoAR 2.0 features outperforms the model trained on the full 960-hour dataset with filterbank features.

==> decoar 2.0/01_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Automatic speech recognition (ASR) systems are typically trained on vast quantity of paired audio and text data to attain competitive performance. Obtaining these paired data requires substantial human annotation efforts and is often time-consuming, expensive and error-prone. With the emerging popularity of end-to-end ASR models, the need for large amounts of training data is more demanding than the conventional hybrid-based ASR systems. For this purpose, semi-supervised learning (SSL) is often investigated for speech recognition, where a model is trained using a finite amount of labeled data and a much larger amount of unlabeled data. 

In the long history of semi-supervised learning (SSL) in speech recognition, self-training approach \cite{vesely2013semi,huang2016semi,synnaeve2019end} and knowledge distillation \cite{hinton2015distilling}, or known as teacher-student model training \cite{li2014learning} are the two commonly used SSL methods. Recent success of representation learning enables a new approach towards leveraging unlabeled data. In natural language processing community,  BERT~\cite{devlin2019bert}, ELMo~\cite{peters2018deep}, XLNet \cite{yang2019xlnet}, GPT  \cite{radford2018improving} and its follow-ups are classical examples of representation learning. The key philosophy of representation learning is based on using self-supervised learning, where we obtain `free' labels from unlabeled data and train them in a supervised manner via some proxy tasks. In the context of BERT~\cite{devlin2019bert}, two proxy tasks are defined including masked language model task and two-sequence prediction task. These proxy tasks are designed to force the learning of a robust, meaningful representation.  After the representation has been learned, a downstream task model is then trained using labeled data with the learned representation. Optionally, the representation learning block and downstream task block can be fine-tuned together. 

Learning efficient speech representation can be traced back to restricted Boltzmann machine \cite{hinton2006fast, hinton2012deep, bengio2007greedy}, which allows pre-training on large amounts of unlabeled data before training the deep neural network speech models.  More recently, speech representation learning has drawn increasing attention in speech processing community and has shown promising results in semi-supervised speech recognition \cite{schneider2019wav2vec, baevski2020wav2vec, ling2020deep, liu2020tera}.  The design of proxy tasks in learning speech representation can be categorized into two types. The first type is based on \textbf{contrastive loss}~\cite{van2017neural} and has been applied to speech representation such as wav2vec and its variants \cite{schneider2019wav2vec,baevski2019vq,baevski2020wav2vec}. The model is trained to learn representations containing information that most discriminates the future or masked frame from a set of negative samples via contrastive loss.  The second type is based on \textbf{reconstructive loss}. The proxy task for these representation learning methods is to reconstruct temporal slices of acoustic features based on contextual information. These reconstruction tasks can be defined as autoregressive reconstruction, or masked-based reconstruction. APC \cite{chung2019unsupervised} and its follow-up \cite{chung2020improved} are examples to use autoregressive reconstruction loss.  In many state-of-the-art pretrained language model task, masked-based prediction is adopted in the proxy tasks such as BERT \cite{devlin2019bert} and XLNet \cite{yang2019xlnet}.  In speech, instead of prediction, we randomly mask temporal slices of acoustic features and attempt to reconstruct them \cite{jiang2019improving, song2019speech, wang2020unsupervised, liu2020mockingjay, chi2020audio, liu2020tera}.

Orthogonal to the contrastive-/reconstructive-loss based speech representation learning, vector-quantized speech representations have been proposed~\cite{van2017neural, liu2020towards, baevski2019vq, baevski2020wav2vec, chung2020vector}. One motivation to apply vector quantization (VQ) is that enforcing quantization can lead to better linguistic unit discovery \cite{oord2018representation, harwath2019learning} due to the discrete nature of phonetic units. In VQ-APC \cite{chung2020vector}, the authors use VQ as a way to limit model capacity and control information needed in encoding representation. In VQ-wav2vec \cite{baevski2019vq} and wav2vec 2.0 \cite{baevski2020wav2vec}, the author use VQ to facilitate direct application of BERT and other NLP algorithms.

In this paper, we introduce DeCoAR 2.0, a \textbf{De}ep \textbf{Co}ntextualized \textbf{A}coustic \textbf{R}epresentation with vector quantization. We take inspirations from many recent advances in speech representation learning, and propose multiple improvements over vanilla DeCoAR. We summarize the contributions of this paper as follows:
\begin{itemize}[leftmargin=*,itemsep=0pt, topsep=1pt]
    \item We propose to use Transformer as encoding block and replace LSTM in the vanilla DeCoAR;
    \item We present a deep contextualized acoustic representation learning approach with the addition of a vector quantization layer;
    \item We propose a new objective function that combines masked-based reconstruction loss with VQ diversity loss.
\end{itemize}

% The rest of the paper is organized as follows. Section~\ref{sec:related} gives a brief overview of our previous DeCoAR method and related work in vector quantized speech representation learning. Section~\ref{sec:approach} describes the proposed DeCoAR 2.0 approach. Experimental results on semi-supervised speech recognition are presented in Section~\ref{sec:expt} followed by conclusion in Section~\ref{sec:conclusion}.


% Learning robust speech representation has been exploited in recent years. Among these approaches, wav2vec 2.0 \cite{baevski2020wav2vec} uses 10 minutes of labeled data with 53k hours of unlabeled data to achieve a word error rate (WER) of 5.2/8.6 on LibriSpeech benchmark. The model relies on a diverse codebook learnt to correlates the underlying speech units to speech representations via the contrastive loss. However, the contrastive loss formulation can result in several locally optimal codebooks, for exmaples, acoustic condition-sensitive codebooks: where the model can easily optimized by assign acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporally invariant codebooks: where the model assigns specific codes to fixed temporal locations. 

%Furthermore, the codes at each time step the model select right after their feature encoder hardly contained meaningful phonetic information. So their contrastive approach might not generalize well to all datasets, espically the real world data consisted a lot of nausence factor like noise, different recording environment. 

% A simple workaround could be using frame reconstruction as objective, the network allows a flow of information from the input feature back to the the latent space to preserve meaningful information in the codes, helping mitigatate the codebook learning problems in contrastive loss as discussed above. And compared to simple reconstruction where we utilize all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. By utilizing the VQ layer, the model is able to keep the representation from those unwanted information flowing. 



% Automatic speech recognition (ASR) systems are typically trained on vast quantity of paired audio and text data to attain competitive performance. Obtaining these paired data requires substantial human annotation efforts and is often time-consuming, expensive and error-prone. With the emerging popularity of end-to-end ASR models, the need for large amounts of training data is more demanding than the conventional hybrid-based ASR systems. For this purpose, semi-supervised learning (SSL) is often investigated for speech recognition, where a model is trained using a finite amount of labeled data and a much larger amount of unlabeled data. 

% In the long history of SSL in speech recognition, self-training approach \cite{vesely2013semi,huang2016semi,synnaeve2019end} is the most commonly used approach. In self-training methods, a `seed' ASR model is trained using paired audio/text data. The resulting model is then applied to transcribe the unlabeled audio data. The resulting hypotheses, combined with different data selection criteria, are treated as `pseudo-labels' and added to the original labeled dataset to retrain a new model. Simple in concept, self-training works well in practice with one major caveat - the pseudo-label injects systematic bias introduced by the seed model. To alleviate this, careful confidence calibration with system combinations are often used \cite{huang2013semi}. Another family of SSL is based on knowledge distillation \cite{hinton2015distilling}, or teacher-student model training \cite{li2014learning}, and is mostly applied to acoustic model training in hybrid-based ASR. In these setups, a teacher model  generates frame-wise soft label instead of hard label, and a student model is trained on the soft labels via KL divergence loss instead of a standard cross-entropy loss based on forced alignment. The knowledge distillation based SSL partially mitigates the systematic bias but is rarely being investigated towards sequence-level loss \cite{wong2016sequence,manohar2018semi} or end-to-end ASR systems. 


% Recent success of efficient representation learning, in particular in natural language processing (NLP), enables a new approach towards leveraging unlabeled data. Classical examples of representation learning for NLP include BERT~\cite{devlin2019bert}, ELMo~\cite{peters2018deep}, XLNet \cite{yang2019xlnet}, GPT and its follow-ups \cite{radford2018improving}, to name but a few.  The key philosophy of representation learning is based on self-supervised learning, where we obtain `free' labels from unlabeled data and train them in a supervised manner via some proxy tasks. In the context of the well-known BERT~\cite{devlin2019bert}, two proxy tasks are defined including masked language model task and two-sequence prediction task. These proxy tasks are defined in a way to force the learning of a robust, meaningful representation.  A downstream task is then trained on the labeled data with the learned representation. Optionally, the representation learning block and downstream task can be fine-tuned together. 



% This paper presents DeCoAR 2.0, a follow-up on DeCoAR \cite{ling2020deep}. We take inspiration from many recent advances in speech representation learning, and propose multiple improvements over vanilla DeCoAR. We summarize the contributions of this paper as follows:
% \begin{itemize}[leftmargin=*,itemsep=0pt, topsep=1pt]
%     \item We propose to use Transformer as encoding block and replace LSTM in vanilla DeCoAR;
%     \item We use BERT-style masked-based reconstruction loss as opposed to autoregressive reconstruction loss in vanilla DeCoAR;
%     \item We present a vector quantized deep contextualized acoustic representation learning approach with the addition of a vector quantization layer;
% \end{itemize}

% The rest of the paper is organized as follows. Section~\ref{sec:related} gives an overview on related work in speech representation learning, and a brief recap of our previous DeCoAR method. Section~\ref{sec:approach} describes the proposed vector quantized DeCoAR approach. Experimental results on semi-supervised speech recognition are presented in Section~\ref{sec:expt} followed by conclusion in Section~\ref{sec:conclusion}.


% In this work, we propose an improved speech representation learning paradigms towards semi-supervised speech recognition based on our previous work \cite{ling2020deep}.


% Current state-of-the-art models for speech recognition require vast amounts of transcribed audio data to attain good performance. In particular, end-to-end ASR models are more demanding in the amount of training data required when compared to traditional hybrid models. While obtaining a large amount of labeled data requires substantial effort and resources, it is much less costly to obtain abundant unlabeled data. 

% For this reason, \textit{semi-supervised learning} (SSL) is often used when training ASR systems. Recently, self-supervised learning—a paradigm that treats the input itself or modifications of the input as learning targets— has obtained promising results. Those self-supervised speech representation can be fall into main categories: Contrastive Predictive Coding \cite{schneider2019wav2vec, baevski2019vq, baevski2020wav2vec} incorporates contrastive objective to learn representations containing information that  most discriminates the future or masked frame from a set of negative samples. Another approach is Autoregressive Predictive Coding (APC) \cite{chung2019unsupervised, liu2020mockingjay, chung2020vector, ling2020deep, wang2020unsupervised}, which tries to directly predict or reconstruct the frame based on context.

% More recently, vector-quantized representations of audio data has drawn increasing attention in speech processing \cite{van2017neural, liu2020towards, baevski2020wav2vec, chung2020vector}. The motivation is that enforcing the quantization leads to a better representation for acoustic unit discovery due to the discrete nature of phonetic units. VQ-APC \cite{chung2020vector} also try to exactly quantified of information (i.e., bits required to transmit the codebook and the sequence of codes), to control the capacity of the models. And the use of vector quantization limited capacity are forced to retain information to achieve maximal prediction. 

% Despite the success of the wav2vec 2.0 model \cite{baevski2020wav2vec}, the model relies on a diverse codebook learnt to correlates the underlying speech units to speech representations via the contrastive loss. However, the codes at each time step the model select right after feature encoder hardly contained meaningful phonetic information. More importantly, contrastive loss formulation can result in several locally optimal codebooks. A few highly probable optima observed were acoustic condition-sensitive codebooks: where the model can easily optimized by assign acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporally invariant codebooks: where the model assigns specific codes to fixed temporal locations to enable a good contrastive loss. Hence, the codebook learning methodology using contrastive loss might not generalize well to all datasets, espically the real world data consisted a lot of nausence factor like noise, different recording environment.  

% A simple solution could be to enforce the codes to explicitly carry information about the input features in the process. Using frame reconstruction as objective, the network allows a flow of information from the input feature back to the the latent space to preserve meaningful information, helping mitigatate the codebook learning problems in contrastive loss as discussed above. Thus, we propose an novel self-supervised model that learns vector quantized deep transformer acoustic representations based on frames reconstruction. Since simple reconstruction utilize all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. And by utilizing the VQ layer to limit those unwanted information flow into final representation, Vector Quantized Deep Contextualized Acoustic Representations (DeCoAR 2.0) are able to achieve much better representation that's better suited for semi-supervised ASR tasks. By using a large amount of unlabeled data, and then applies these representations to ASR tasks using a limited amount of labeled data. In our implementation, we perform acoustic representation learning using deep transformer and a training objective that minimizes the reconstruction error of a temporal slice of filterbank features given context frames. After pre-training, we fix these parameters and add output layers with connectionist temporal classification (CTC) loss for the ASR task. We only train the small ASR model instead of fine-tuning for computing-efficiency. Our approach showed that supervision with 10 hours of labeled data on DeCoAR 2.0 achieves performance on par with training on all 960 hours directly.

==> decoar 2.0/02_related.tex <==
\section{Related Work}
\label{sec:related}

% \subsection{Speech Representation Learning}

% Learning efficient acoustic representation can be traced back to restricted Boltzmann machine \cite{hinton2006fast, hinton2012deep, bengio2007greedy}, which allows pre-training on large amounts of unlabeled data before training the deep neural network acoustic models.  More recently, acoustic representation learning has drawn increasing attention  \cite{hsu2018extracting, chung2019unsupervised, chorowski2019unsupervised, schneider2019wav2vec, pascual2019learning, baevski2019vq, baevski2020wav2vec} in speech processing and has shown promising results in semi-supervised speech recognition.  As mentioned in the introduction, the key to a robust representation learning is the design of the proxy supervised task.  Most proxy tasks in acoustic representation learning can fall into two categories. 

% The first one is based on \textbf{contrastive loss}~\cite{van2017neural} and has been applied to speech representation such as wav2vec and its variants \cite{schneider2019wav2vec,baevski2019vq,baevski2020wav2vec}. To train acoustic representation with contrastive loss, an encoder network maps the original acoustic features (MFCCs, fiterbanks) into a latent space. A context network maps multiple latent representations into a contextualized representation. The model is trained to learn representations containing information that most discriminates the future or masked frame from a set of negative samples via contrastive loss.  

% The second one is based on \textbf{reconstructive loss}. The proxy task for these representation learning methods is to reconstruct temporal slices of acoustic features. These reconstruction tasks can be defined as autoregressive reconstruction, or masked-based reconstruction. APC \cite{chung2019unsupervised} and its follow-up \cite{chung2020improved} are examples to use autoregressive reconstruction loss.  In many state-of-the-at pretrained language model task, masked-based prediction is adopted in the proxy tasks such as BERT \cite{devlin2019bert} and XLNet \cite{yang2019xlnet}.  In speech, instead of prediction, we randomly mask slices of acoustic features and attempt to reconstruct them. \cite{jiang2019improving, song2019speech, wang2020unsupervised, liu2020mockingjay, chi2020audio, liu2020tera}.

% For example, an autoregressive predictive coding model (APC) was proposed in \cite{chung2019unsupervised} for unsupervised speech representation learning and was applied to phone classification and speaker verification. WaveNet auto-encoders \cite{chorowski2019unsupervised} proposed contrastive predictive coding (CPC) to learn speech representations and was applied on unsupervised acoustic unit discovery task. Wav2vec~\cite{schneider2019wav2vec} proposed a multi-layer convolutional neural network optimized via a noise contrastive binary classification and was applied to WSJ ASR tasks. As its follow-up work\cite{baevski2020wav2vec}, Wav2vec-2.0 is introduced where the contrastive task is defined over a quantized latent representation. It was shown by training acoustic representation over 53,000-hour unlabeled audio data, they were able to attain competitive performance on LibriSpeech using only 10 minutes of labeled data. Similar idea has also been exploited to the APC model, where a vector-quantized APC model was proposed\cite{chung2020vector}.


\subsection{An Overview on DeCoAR}

DeCoAR stands for \textit{deep contextualized acoustic representations}, and was proposed in our previous work~\cite{ling2020deep}. As depicted in Figure~\ref{fig:decoar}, DeCoAR consists of two modules, an encoder module and a reconstruction module. For an input speech sequence $\mathbf{X} = (\mathbf{x}_1,\cdots,\mathbf{x}_T)$, an \textbf{encoder module} consists of a stacked forward and backward LSTMs, and computes a hidden representation that encodes information from both previous and future frames (i.e. $\overrightarrow{\mathbf{z}}_t, \overleftarrow{\mathbf{z}}_t$). For each temporal slice $(\mathbf{x}_t, \mathbf{x}_{t+1}, ..., \mathbf{x}_{t+K})$, the \textbf{reconstruction module} takes the concatenated forward state at time $t$ and backward state at $t+K$ as inputs, and uses  position-dependent feed-forward networks to recontruct each frame. Formally, the DeCoAR objective is defined as follows:
\begin{equation}\label{eq:decoar}
  \begin{aligned}
\mathcal{L}_t= \sum_{i=0}^{K}|\mathbf{x}_{t+i} - \text{FFN}_i ([\overrightarrow{\mathbf{z}}_t; \overleftarrow{\mathbf{z}}_{t+K}])|
\end{aligned}
\end{equation}
where $\text{FFN}_i$ is a position-dependent feed-forward network to reconstruct the $i$-th frame in the slice.  The final loss $\mathcal{L}$ is calculated over all possible slices in the entire sequence in an autoregressive manner, defined as: $\mathcal{L}=\sum_{t=1}^{T-K}\mathcal{L}_t$.

\begin{figure}[th]
  \centering
  \includegraphics[width=0.9\linewidth]{decoar_icassp2021.pdf}
  \caption{Illustration of DeCoAR.}
  \label{fig:decoar}
\end{figure}

\subsection{Vector-quantized Representation Learning}
\subsubsection{wav2vec 2.0}
Wav2vec 2.0 \cite{baevski2020wav2vec} is one of the successful examples in representation learning. It uses 10 minutes of labeled data with 53k hours of unlabeled data to achieve a word error rate (WER) of 5.2\%/8.6\% on LibriSpeech benchmark. The model relies on a diverse codebook learned to correlate the underlying speech units to representations via contrastive loss. Discretizing the continuous representation enables applications of many state-of-the-art NLP algorithms. In wav2vec 2.0, after applying VQ operations, the model is trained using a masked LM style loss, similar to BERT. 

One potential challenge in learning optimal codebooks with contrastive loss is posed by data with nuisance factors such as noise and other adverse conditions. In these cases, the codebook can be trivially optimized by assigning acoustic condition (e.g. voice activity, noise) to the codebook. A potential work-around is to use frame reconstruction as objective so that the network can leverage all available information of the input feature to guide the learning of a robust representation. %Another solution is to perform vector quantization operation at a higher layer (closer to final output layer), as opposed to a lower layer. 
% flow back to the the codes to preserve meaningful information, helping mitigate the codebook learning problems in contrastive loss as discussed above.

% However, contrastive loss formulation can result in several locally optimal codebooks. For examples, acoustic condition-sensitive codebooks in which the model can easily be optimized by assigning acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporal codebooks in which the model assigns specific codes to fixed temporal locations for a minimum contrastive loss. Thus, this codebook learning methodology using contrastive loss may not generalize well to all datasets, especially the real world data contained a lot of nuisance factor like noise, adverse environment.  A simple work-around is to use frame reconstruction as objective, so the network allows information of the input feature flow back to the the codes to preserve meaningful information, helping mitigate the codebook learning problems in contrastive loss as discussed above.

\subsubsection{VQ-APC}
VQ-APC \cite{chung2020vector} introduced an novel approach that inserted a VQ layer before frame prediction. The motivation of using VQ is to quantify the information needed to encode speech representation and control the capacity of the models. The model uses autoregressive predictive coding (APC) as objective, instead of a contrastive predictive coding (CPC). Their experiments showed APC/reconstruction objective performed better than CPC/constrastive objective under the same condition. They also demonstrated the learned VQ codes highly correlate to phoneme path, suggesting VQ can be used to capture linguistic units in an implicit way. 
% Since direct prediction make the model to utilize all the information available (phonetics, speaker traits, background noise, etc.) to achieved maximal prediction. While most of those information are not important to ASR and also made the task complicated. And by utilizing the VQ layer to limit the capacity, the model is able to focus on only a few certain information. Their experiment also showed that APC objective performed better than CPC objective under the same condition.


\begin{figure*}[thb]
  \centering
  \includegraphics[width=0.8\linewidth]{decoar2_2fig.pdf}
  \caption{Illustration of DeCoAR 2.0 framework. The left side shows the architecture of speech representation model using unlabeled data. The right side shows an example on using labeled data with the learned speech representation. Note that the quantization and reconstruction modules are removed, and a frozen encoder is attached to a downstream ASR model (such as an acoustic model in hybrid-based system, or an end-to-end ASR system). Only the parameters in ASR model block are trained. }
  \label{fig:model_view}
\end{figure*}
% \subsection{Vector-quantized Representation Learning}

% Orthogonal to the contrastive-/reconstructive-loss based representation learning, vector-quantized representations of audio data has been proposed~\cite{van2017neural, liu2020towards, baevski2020wav2vec, chung2020vector}. The motivation is that enforcing the quantization leads to a better representation for acoustic unit discovery due to the discrete nature of phonetic units. VQ-APC \cite{chung2020vector} also try to exactly quantified of information (i.e., bits required to transmit the codebook and the sequence of codes), to control the capacity of the models \yuzong{Rewrite this}. And the use of vector quantization limited capacity are forced to retain information to achieve maximal prediction. 



% Despite the success of the wav2vec 2.0 model \cite{baevski2020wav2vec}, the model relies on a diverse codebook learnt to correlates the underlying speech units to speech representations via the contrastive loss. However, the codes at each time step the model select right after feature encoder hardly contained meaningful phonetic information. More importantly, contrastive loss formulation can result in several locally optimal codebooks. A few highly probable optima observed were acoustic condition-sensitive codebooks: where the model can easily optimized by assign acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporally invariant codebooks: where the model assigns specific codes to fixed temporal locations to enable a good contrastive loss. Hence, the codebook learning methodology using contrastive loss might not generalize well to all datasets, espically the real world data consisted a lot of nausence factor like noise, different recording environment.  

% A simple solution could be to enforce the codes to explicitly carry information about the input features in the process. Using frame reconstruction as objective, the network allows a flow of information from the input feature back to the the latent space to preserve meaningful information, helping mitigatate the codebook learning problems in contrastive loss as discussed above. Thus, we propose an novel self-supervised model that learns vector quantized deep transformer acoustic representations based on frames reconstruction. Since simple reconstruction utilize all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. And by utilizing the VQ layer to limit those unwanted information flow into final representation, Vector Quantized Deep Contextualized Acoustic Representations (DeCoAR 2.0) are able to achieve much better representation that's better suited for semi-supervised ASR tasks. By using a large amount of unlabeled data, and then applies these representations to ASR tasks using a limited amount of labeled data. In our implementation, we perform acoustic representation learning using deep transformer and a training objective that minimizes the reconstruction error of a temporal slice of filterbank features given context frames. After pre-training, we fix these parameters and add output layers with connectionist temporal classification (CTC) loss for the ASR task. We only train the small ASR model instead of fine-tuning for computing-efficiency. Our approach showed that supervision with 10 hours of labeled data on DeCoAR 2.0 achieves performance on par with training on all 960 hours directly.


% to reconstruct each frame in the original slice. 

% for each slice starting at time $t$ and ending at $t+K$. The reconstruction module takes the $\overrightarrow{\mathbf{z}}_t, \overleftarrow{\mathbf{z}}_t$ and aims at reconstructing each frame 

% DeCoAR falls into the category of \textbf{reconstructive loss} based approach.  We train the DeCoAR model to predict a \textit{slice} of acoustic feature vectors, given past and future acoustic vectors. As depicted on the left side of Figure~\ref{fig:decoar}, a stack of forward and backward LSTMs are applied to the entire unlabeled input sequence $\mathbf{X} = (\mathbf{x}_1,\cdots,\mathbf{x}_T)$, where the $\mathbf{x}_t$ are 40-dimensional log filterbank features. The encoder network computes a hidden representation that encodes information from both previous and future frames (i.e. $\overrightarrow{\mathbf{z}}_t, \overleftarrow{\mathbf{z}}_t$) for each frame $\mathbf{x}_t$.  Given a sequence of acoustic feature inputs  $(\mathbf{x}_1, ..., \mathbf{x}_{T}) \in \mathbb{R}^d$, for each slice $(\mathbf{x}_t, \mathbf{x}_{t+1}, ..., \mathbf{x}_{t+K})$ starting at time step $t$, our objective is defined as follows:
% \begin{equation}\label{eq:decoar}
%   \begin{aligned}
% \mathcal{L}_t= \sum_{i=0}^{K}|\mathbf{x}_{t+i} - \text{FFN}_i ([\overrightarrow{\mathbf{z}}_t; \overleftarrow{\mathbf{z}}_{t+K}])|
% \end{aligned}
% \end{equation}
% where $[\overrightarrow{\mathbf{z}}_t; \overleftarrow{\mathbf{z}}_{t}] \in \mathbb{R}^{2h}$ are the concatenated forward and backward states from the last LSTM layer, and
% \begin{equation}
%     \text{FFN}_i(\mathbf{v}) = \mathbf{W}_{i,2} \text{ReLU}(\mathbf{W}_{i,1} \mathbf{v} + \mathbf{b}_{i,1})  + \mathbf{b}_{i,2}
% \end{equation}
% is a position-dependent feed-forward network with 512 hidden dimensions. The final loss $\mathcal{L}$ is summed over all possible slices in the entire sequence:
% \begin{equation}
%   \begin{aligned}
% \mathcal{L}=\sum_{t=1}^{T-K}\mathcal{L}_t
% \end{aligned}
% \end{equation}

% DeCoAR consists of two modules, a encoder network that encodes a temporal slice of filterbank features 

% To train DeCoAR, a deep bi-directional LSTM network encodes a temporal slice of filterbank features into a latent feature space 



% In our previous work \cite{ling2020deep}, we proposed a different perspective towards semi-supervised speech recognition via representation learning. First, a large amount of unlabeled data is used to train robust acoustic representation by reconstructing temporal slices of filterbank features from past and future context frames in an autoregressive way. This acoustic representation is referred to as \textit{deep contextualized acoustic representations}, or DeCoAR in short. The labeled data is then applied with the DeCoAR, which is used to train an ASR system. We observed highly comparable performance using limited amount of the labeled data using DeCoAR compared to using the entire 960-hour conventional filterbank features on LibriSpeech dataset. 

% In speech recognition, similar ideas have been investigated.  Those self-supervised speech representations fall into these categories: \textbf{Contrastive Predictive Coding} \cite{schneider2019wav2vec, baevski2019vq, baevski2020wav2vec} incorporates contrastive objective to learn representations containing information that  most discriminates the future or masked frame from a set of negative samples. Another approach is \textbf{Autoregressive Predictive Coding (APC)} \cite{chung2019unsupervised, liu2020mockingjay, chung2020vector, ling2020deep, wang2020unsupervised}, which tries to directly predict or reconstruct the frame based on context.

% More recently, vector-quantized representations of audio data has drawn increasing attention in speech processing \cite{van2017neural, liu2020towards, baevski2020wav2vec, chung2020vector}. The motivation is that enforcing the quantization leads to a better representation for acoustic unit discovery due to the discrete nature of phonetic units. VQ-APC \cite{chung2020vector} also try to exactly quantified of information (i.e., bits required to transmit the codebook and the sequence of codes), to control the capacity of the models. And the use of vector quantization limited capacity are forced to retain information to achieve maximal prediction. 

% % Despite the success of the wav2vec 2.0 model \cite{baevski2020wav2vec}, the model relies on a diverse codebook learnt to correlates the underlying speech units to speech representations via the contrastive loss. However, the codes at each time step the model select right after feature encoder hardly contained meaningful phonetic information. More importantly, contrastive loss formulation can result in several locally optimal codebooks. A few highly probable optima observed were acoustic condition-sensitive codebooks: where the model can easily optimized by assign acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporally invariant codebooks: where the model assigns specific codes to fixed temporal locations to enable a good contrastive loss. Hence, the codebook learning methodology using contrastive loss might not generalize well to all datasets, espically the real world data consisted a lot of nausence factor like noise, different recording environment.  

% A simple solution could be to enforce the codes to explicitly carry information about the input features in the process. Using frame reconstruction as objective, the network allows a flow of information from the input feature back to the the latent space to preserve meaningful information, helping mitigatate the codebook learning problems in contrastive loss as discussed above. Thus, we propose an novel self-supervised model that learns vector quantized deep transformer acoustic representations based on frames reconstruction. Since simple reconstruction utilize all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. And by utilizing the VQ layer to limit those unwanted information flow into final representation, Vector Quantized Deep Contextualized Acoustic Representations (DeCoAR 2.0) are able to achieve much better representation that's better suited for semi-supervised ASR tasks. By using a large amount of unlabeled data, and then applies these representations to ASR tasks using a limited amount of labeled data. In our implementation, we perform acoustic representation learning using deep transformer and a training objective that minimizes the reconstruction error of a temporal slice of filterbank features given context frames. After pre-training, we fix these parameters and add output layers with connectionist temporal classification (CTC) loss for the ASR task. We only train the small ASR model instead of fine-tuning for computing-efficiency. Our approach showed that supervision with 10 hours of labeled data on DeCoAR 2.0 achieves performance on par with training on all 960 hours directly.

==> decoar 2.0/03_method.tex <==
\section{Proposed Framework}
\label{sec:approach}

DeCoAR 2.0 is a follow-up work based on DeCoAR, and we take inspirations of recent advancement in natural language and speech representation learning.  The left figure in Figure~\ref{fig:model_view} illustrates the proposed DeCoAR 2.0 architecture. The model consists of three modules. The first module is the \textbf{encoder network} that maps input masked acoustic frames $\mathbf{x}_{t+1},\cdots,\mathbf{x}_{t+K}$ into a latent representation $\mathbf{z}_{t+1},\cdots,\mathbf{z}_{t+K}$ via multiple Transformer blocks. The second module is the \textbf{vector quantization network} that maps latent representation $\mathbf{z}_{t+1},\cdots,\mathbf{z}_{t+K}$ to a new quantized representation $\mathbf{v}_{t+1},\cdots,\mathbf{v}_{t+K}$. The last module, \textbf{reconstruction network}, takes the quantized representation to a feed-forward network and reconstructs the original input frames as $\mathbf{y}_{t+1},\cdots,\mathbf{y}_{t+K}$. We will describe the design of each module and its training criterion in the following sections.

\subsection{Encoder Module}
We replace forward/backward LSTM with Transformer,  due to its superiority in modeling long context \cite{vaswani2017attention,wang2020transformer}. While RNN/LSTM can model long context in theory, the Transformer achieves better performance thanks to its multi-head attention mechanism that captures the relationship for any arbitrary pair of samples in a long input sequence. In our encoder, we use a 1D convolutional layer with kernel size of 256 and 16 groups. This performs an implicit relative positional encoding as pointed out in \cite{mohamed2019transformers}. The convolution is followed by Gaussian Error Linear Unit (GELU) and layer normalization. The output is then fed into the deep transformer encoder network and produce a sequence of hidden vectors $\mathbf{Z} = (\mathbf{z}_1,\cdots,\mathbf{z}_T)$. 

In our masking strategy, we mask a proportion of the feature and replace them with a trainable feature vector. We randomly mask the subsequent $K$ consecutive time steps from every sampled index; spans are not overlap and we masked around 40\% frames in total.

\subsection{Quantization Module}

We introduce a quantization module in DeCoAR 2.0 framework. Quantization module takes the latent representation $\mathbf{z}_t$ from encoder module, and map it to a new representation $\mathbf{v}_t$. This is done by selecting one entry from a fixed-size codebook $C=\{c_1, \cdots, c_V\}$, where $V$ is the size of the codebook, and apply a linear transformation to obtain $\mathbf{v}_t$. Selecting an entry in a discrete cookbook is not differentiable. To mitigate the problem, we use the Gumbel-Softmax loss with reparameterization trick.  In line with VQ-wav2vec \cite{baevski2019vq}, wav2vec 2.0 \cite{baevski2020wav2vec} and VQ-APC \cite{chung2020vector}, we use the straight-through Gumbel-Softmax estimator~\cite{jang2017categorical}. 

In our quantization module, we use multiple codebooks \cite{baevski2020wav2vec} to obtain quantized representations.  Formally, given the latent representation $\mathbf{z}$ from the encoder module, a set of codebooks $C_1, \cdots, C_G$ where $G$ is the number of codebooks, $V$ entries in each codebook, we select one variable from each codebook and stack the resulting vectors followed by a linear transformation to obtain new representation $\mathbf{v}$. In order to train which entry to select, we map the encoder output $\mathbf{z}$ to logits $\mathbf{l}\in\mathcal{R}^{G\times V}$ via a linear layer, and the probability of selecting the $j$-th code in $g$-th codebook is defined as follows:
\begin{equation}\label{eq:gumble}
  \begin{aligned}
p_{g, j}=\frac{\exp(\mathbf{l}_{g,j}+n_j)/\tau}{\sum_{k=1}^{V}\exp(\mathbf{l}_{g,k}+n_k)/\tau}
\end{aligned}
\end{equation}
where $\tau> 0$ is the softmax temperature, $n=-\ln(-\ln(u))$ and $u$ are uniformly sampled from $\mathcal{U}(0,1)$. In inference, the index with largest value in logits $\mathbf{l}$ is selected from each codebook. 

% we apply a linear transformation to map it to a vector $\mathbf{l}\in \mathcal{R}^{G\times V}$. During inference, the index $j=\text{argmax}_i(\mathbf{l}_{g,i})$ is selected.  During training, the probability of selecting the $j$-th code for group g is defined as follows:
% \begin{equation}\label{eq:gumble}
%   \begin{aligned}
% p_{g, j}=\frac{\exp(\mathbf{l}_{g,j}+n_j)/\tau}{\sum_{k=1}^{V}exp(\mathbf{l}_{g,k}+n_k)/\tau}
% \end{aligned}
% \end{equation}
% where $n=−ln(−ln(u))$ and $u$ are uniformly sampled from $\mathcal{U}(0,1)$. $\tau$ controls  how  close  the approximation is to argmax.

% % As shown in VQ-APC \cite{chung2020vector}, the authors observed the VQ-APC models with multiple vector quantization layers have trouble fitting the training set and they concluded that inserting VQ layer after encoder modules works in practice. We follow their setting and add the VQ layer after the transformer encoder blocks. 

% We use the Gumbel-Softmax with the straight-through estimator for selecting discrete codebook variables in a fully differentiable way. Specifically, we apply a linear layer to map z to vectors belongs to the V codebooks. 

% At test time, we simply choose the largest index.  At training time, the probability $p_i$ of selecting the i-th code for group g as follows:
% \begin{equation}\label{eq:gumble}
%   \begin{aligned}
% p_{g,v}=\frac{exp(l_{g,v}+n_v)/\tau}{\sum_{k=1}^{V}exp(l_{g,k}+n_k)/\tau}
% \end{aligned}
% \end{equation}

% where $v=−ln(−ln(u))$ uniformly  sampled  from $U(0,1)$. $\tau$ controls  how  close  the approximation is to argmax. During  the  forward  pass,  the  argmax  codec k where $k=argmax_i(p_i)$ is chosen;  during the backward pass, the true gradients of the Gumbel-Softmax outputs are used. 

\subsection{Training Objective}

The training objective consists of two parts. The first objective is the \textbf{reconstruction loss}. We use $\ell_1$ loss between an acoustic feature vectors $\mathbf{X}$ at time $t$ and a reconstruction $\mathbf{Y}$  predicted at time $t$ for all masked indices $t$, defined as $\mathcal{L}_{recon}=\sum_t|\mathbf{x}_{t} - \mathbf{y}_t|$. We use $\ell_1$ loss as it is less sensitive to outliers.
% \begin{equation}\label{eq:recon}
%   \begin{aligned}
% L_{recon}=\sum_t|\mathbf{x}_{t} - \mathbf{y}_t|
% \end{aligned}
% \end{equation}

Since vector quantization layers are known to significantly disrupt model training, we apply the \textbf{diversity loss} proposed in wav2vec 2.0 \cite{baevski2020wav2vec} to encourage the equal use of all entries in each codebook. Diversity loss maximizes the entropy of the averaged softmax distribution over the entries for each codebook in each mini-batch. Formally, the \textbf{diversity loss} is defined as: 
% $L_{div}=\frac{1}{GV}\sum_{g=1}^{G}\sum_{v=1}\bar{p}_{gv}log\bar{p}_{gv}$
\begin{equation}\label{eq:div} 
  \begin{aligned}
\mathcal{L}_{div}= \frac{GV-\sum_{g=1}^G \exp(-\sum_{v=1}^V p_{g,j} \log p_{g,j})}{GV} % \frac{1}{GV}\sum_{g=1}^{G}\sum_{v=1}\bar{p}_{gv}log\bar{p}_{gv}
\end{aligned}
\end{equation}

Our final training objective is a combination of the two loss functions, weighted by a hyperparameter $\alpha$:
\begin{equation}\label{eq:loss}
  \begin{aligned}
\mathcal{L}=\mathcal{L}_{recon}+\alpha \mathcal{L}_{div}
\end{aligned}
\end{equation}


\subsection{Semi-supervised Speech Recognition with DeCoAR 2.0}

After we have pre-trained the DeCoAR 2.0 model on unlabeled data, we freeze all the parameters in the network. We remove the quantization module and reconstruction module. The representations from the Transformer encoder module are then attached to a downstream ASR system. This ASR system can be either a conventional acoustic model in a hybrid-based ASR system, or an end-to-end speech recognition such as RNN-Transducers \cite{rao2017exploring,li2019improving} or Encoder-Decoder based model \cite{chan2016listen,watanabe2017hybrid}. Note that in our framework, we only train parameters for the downstream ASR model and leave all parameters in the encoder module fixed (i.e. no backpropagation to all layers in encoder module). 


% To train an end-to-end ASR \yuzong{don't say end-to-end. this CTC model a hybrid system indeed} system using labeled data, we remove the reconstruction layer and VQ layer and add two BLSTM layers with CTC loss \cite{graves2016ctc}, as illustrated on the right side of Figure~\ref{fig:model_view}. Since fine-tuning requires retraining all layers, and for computing-efficiency and simplicity, we only train the parameters of this ASR-specific new layer instead of all layers on the labeled data. 

% Furthermore, since VQ-APC \cite{chung2020vector} and wav2vec 2.0 \cite{baevski2020wav2vec} and our model are trained in different toolkit, fine-tuning in different system won't be a fair comparison. So we extract their representation from ASR data in order to use the same ASR toolkit.



% Despite the success of the wav2vec 2.0 model \cite{baevski2020wav2vec}, the model relies on a diverse codebook learnt to correlates the underlying speech units to speech representations via the contrastive loss. However, the codes at each time step the model select right after feature encoder hardly contained meaningful phonetic information. More importantly, contrastive loss formulation can result in several locally optimal codebooks. A few highly probable optima observed were acoustic condition-sensitive codebooks: where the model can easily optimized by assign acoustic condition (e.g. voice activity, noise) to the the codebooks, and temporally invariant codebooks: where the model assigns specific codes to fixed temporal locations to enable a good contrastive loss. Hence, the codebook learning methodology using contrastive loss might not generalize well to all datasets, espically the real world data consisted a lot of nausence factor like noise, different recording environment.  

% A simple solution could be to enforce the codes to explicitly carry information about the input features in the process. Using frame reconstruction as objective, the network allows a flow of information from the input feature back to the the latent space to preserve meaningful information, helping mitigatate the codebook learning problems in contrastive loss as discussed above. Thus, we propose an novel self-supervised model that learns vector quantized deep transformer acoustic representations based on frames reconstruction. Since simple reconstruction utilize all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. And by utilizing the VQ layer to limit those unwanted information flow into final representation, Vector Quantized Deep Contextualized Acoustic Representations (DeCoAR 2.0) are able to achieve much better representation that's better suited for semi-supervised ASR tasks. By using a large amount of unlabeled data, and then applies these representations to ASR tasks using a limited amount of labeled data. In our implementation, we perform acoustic representation learning using deep transformer and a training objective that minimizes the reconstruction error of a temporal slice of filterbank features given context frames. After pre-training, we fix these parameters and add output layers with connectionist temporal classification (CTC) loss for the ASR task. We only train the small ASR model instead of fine-tuning for computing-efficiency. Our approach showed that supervision with 10 hours of labeled data on DeCoAR 2.0 achieves performance on par with training on all 960 hours directly.


% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.9\linewidth]{decoar2.pdf}
%   \caption{Illustration of DeCoAR 2.0 framework.}
%   \label{fig:model_view}
% \end{figure}


% % \begin{figure*}[t]
% %   \centering
% %   \includegraphics[width=0.9\linewidth]{overview.jpg}
% %   \caption{Illustration of our semi-supervised speech recognition system.}
% %   \label{fig:model_view}
% % \end{figure*}


% Figure~\ref{fig:model_view} illustrates the DeCoAR 2.0 architecture. Our model is similar to wav2vec 2.0 \cite{baevski2020wav2vec}. We use 80 dimensional filterbank as our input and is represented as a sequence of acoustic features $\mathbf{X} = (\mathbf{x}_1,\cdots,\mathbf{x}_T)$. We mask a proportion of the feature before feeding them to the model and replace them with a trained feature vector shared between all masked time steps \yuzong{Replace the masked feature with a trained feature???}. We randomly mask the subsequent M consecutive time steps from every sampled index; spans are not overlap and we masked around 40\% frames in total. 

% Then we use a 1D convolutional layer with kernel size 256 and 16 groups similar to which acts as relative positional embedding \cite{mohamed2019transformers}. We add the output of the convolution followed by a GELU and then apply layer normalization. Then the transformer encoder network  produce a sequence of hidden vectors $\mathbf{Z} = (\mathbf{z}_1,\cdots,\mathbf{z}_T)$. Next, we add a vector  quantization layer that replaces $\mathbf{Z}$ with $\mathbf{Z'} = (\mathbf{v}_1,\cdots,\mathbf{v}_T)$, where v is one of the V elements in the codebook ${v_1,...,v_c}$. We then pass the resulting hidden vectors $\mathbf{Z'} = (\mathbf{v}_1,\cdots,\mathbf{v}_T)$ to the the feed-forward layer for reconstruction sequence $\mathbf{Y}=({y_1,...,y_t})$.

% \subsection{Quantization module}
% As shown in VQ-APC \cite{chung2020vector}, the authors observed the VQ-APC models with multiple vector quantization layers have trouble fitting the training set and they concluded that inserting VQ layer after encoder modules works in practice. We follow their setting and add the VQ layer after the transformer encoder blocks. 

% We use the Gumbel-Softmax with the straight-through estimator for selecting discrete codebook variables in a fully differentiable way. Specifically, we apply a linear layer to map z to vectors belongs to the V codebooks. 

% At test time, we simply choose the largest index.  At training time, the probability $p_i$ of selecting the i-th code for group g as follows:
% \begin{equation}\label{eq:gumble}
%   \begin{aligned}
% p_{g,v}=\frac{exp(l_{g,v}+n_v)/\tau}{\sum_{k=1}^{V}exp(l_{g,k}+n_k)/\tau}
% \end{aligned}
% \end{equation}

% where $v=−ln(−ln(u))$ uniformly  sampled  from $U(0,1)$. $\tau$ controls  how  close  the approximation is to argmax. During  the  forward  pass,  the  argmax  codec k where $k=argmax_i(p_i)$ is chosen;  during the backward pass, the true gradients of the Gumbel-Softmax outputs are used. 


% \subsection{Training Objective}
% The model aims to reconstruct original frames from masked frames. So the first objective is to minimize the $\ell_1$ loss between an acoustic feature vectors $\mathbf{X}$ at time $t$ and a reconstruction $\mathbf{Y}$  predicted at time $t$ for all $t$ masked: 

% \begin{equation}\label{eq:recon}
%   \begin{aligned}
% L_{recon}=\sum|\mathbf{x}_{t} - \mathbf{y}_t|
% \end{aligned}
% \end{equation}


% Since vector quantization layers are known to significantly disrupt model training, we use diversity lose describe in \cite{baevski2020wav2vec} to encourage the equal use of the V entries in each of the G codebooks by maximizing the entropy of the averaged softmax distribution over the codebook entries for each codebook:

% \begin{equation}\label{eq:div}
%   \begin{aligned}
% L_d=\frac{1}{GV}\sum_{g=1}^{G}\sum_{v=1}\bar{p}_{gv}log\bar{p}_{gv}
% \end{aligned}
% \end{equation}


% The final objective will be sum over from equation \ref{eq:recon} and equation \ref{eq:div}:
% \begin{equation}\label{eq:loss}
%   \begin{aligned}
% L=L_{recon}+\alpha L_d
% \end{aligned}
% \end{equation}

% where $\alpha$ is a tuned hyperparameter.


% \subsection{End-to-end ASR training with labeled data}

% After we have pre-trained the DeCoAR 2.0 model on unlabeled data, we freeze the parameters in the architecture. To train an end-to-end ASR system using labeled data, we remove the reconstruction layer and VQ layer and add two BLSTM layers with CTC loss \cite{graves2016ctc}, as illustrated on the right side of Figure~\ref{fig:model_view}. Since fine-tuning requires retraining all layers, and for computing-efficiency and simplicity, we only train the parameters of this ASR-specific new layer instead of all layers on the labeled data. 

% Furthermore, since VQ-APC \cite{chung2020vector} and wav2vec 2.0 \cite{baevski2020wav2vec} and our model are trained in different toolkit, fine-tuning in different system won't be a fair comparison. So we extract their representation from ASR data in order to use the same ASR toolkit.



==> decoar 2.0/04_setup.tex <==
\begin{table*}[thb]
    \centering\resizebox{\textwidth}{!}{
   \begin{tabular}{ c | c|cc|cc|cc|cc }
       \toprule
        \multirow{2}{*}{\textbf{Representation}} &
        \multirow{2}{*}{\textbf{Encoder Model}} & \multicolumn{2}{c|}{\textbf{1 hour}} & \multicolumn{2}{c|}{\textbf{10 hours}} & \multicolumn{2}{c}{\textbf{100 hours}} &
        \multicolumn{2}{c}{\textbf{960 hours}}\\
         & &test-clean & test-other & test-clean & test-other & test-clean & test-other &test-clean & test-other\\ 
        \midrule
        filterbank &  - &   50.90 & 78.66 &17.45&  47.18& 9.36 & 30.20  &5.82 &14.50\\
        wav2vec 2.0 \cite{baevski2020wav2vec} & 12 Transformer &  13.63 &29.97 &   5.63& 13.39 & 5.10  & 11.94 &-&- \\
        VQ-APC \cite{chung2020vector}    & 3 uni-GRU                &28.66 & 61.12  & 12.38& 32.28 & 7.42  & 23.38  &-&-  \\
        DeCoAR  \cite{ling2020deep}                    & 4 bi-LSTM &  17.93 &38.38 &  10.40&    27.41&  6.10&17.43  &-&- \\
        DeCoAR 2.0                & 12 Transformer & 13.75 & 29.13 &  5.43& 13.27 & 5.02  & 12.07  &-&-\\
        \bottomrule
    \end{tabular}}
    \caption{Semi-supervised LibriSpeech results. }
    \label{table:LibriSpeech}
\end{table*}

\section{Experimental Setup and Results}
\label{sec:expt}

Our experiments were conducted on the publicly available LibriSpeech dataset. To simulate different SSL scenarios, we varied the labeled data size from 1-hour, 10-hour, up to 100-hour. The 100-hr dataset is based on \textit{train-clean-100} split, and the 1-hr/10-hr subsets are randomly selected from it. 
% We are particularly interested to evaluate the efficacy of the proposed method under data-sparse conditions.  

\subsection{Pretrain DeCoAR 2.0 Model using Unlabeled Data}

To train the DeCoAR 2.0 model, we used the entire 960 hours of LibriSpeech dataset as unlabeled data. We followed the conventional frontend feature extraction, and used a 80-dimensional log-mel filterbank features, which were extracted with a 25ms sliding window at a 10ms frame rate. The features were normalized via mean subtraction and variance normalization on a per-speaker basis. 

For the encoder network in DeCoAR 2.0, we used 12 Transformer blocks, each consists of a multi-head self-attention sublayer followed by a feed forward sublayer. For fair comparison, we set the model dimension to 768, the inner dimension in feed forward sublayer to 3072, with 8 attention heads as used in wav2vec 2.0 base model. The slice size $K$ was set to 20. We optimized the network with Adam and used learning rate warm-up for the first 32000 updates to a peak of 0.0003, and then linearly decayed it. We grouped the input sequences by length with a batch size of 128 (we chopped the maximum length to 15 seconds), and trained the models on 16 GPUs for 150 epochs. The Gumbel softmax temperature $\tau$ is annealed from 2 to a minimum of 0.5 by a factor of $0.999995$ at every update. We use weight $\alpha=0.1$ for the diversity loss and we set $G=2$ and $V=320$ for the quantization module. 


\subsection{Semi-supervised Speech Recognition Experimental Results}

We trained acoustic models using CTC loss on labeled data as downstream tasks. Unlike conventional HMM-based hybrid ASR, training acoustic model with CTC loss gets rid of the need to prepare frame-wise alignments and other tedious processes such as preparing state-tying trees.  The total size of CTC labels were 71 phonemes derived from CMU lexicon, plus one blank symbol. For decoding, we used WFST-based decoding using EESEN \cite{miao2015eesen}. CTC labels, lexicons and a 4-gram language model for LibriSpeech were composed into a WFST-based decoding graph. We set the acoustic model scale to $1.0$, and the blank symbol prior scale to $0.3$. We used \textit{dev-clean} for validation and \textit{test-clean}, \textit{test-other} for evaluation.  

We trained different ASR systems for comparison, using different acoustic representations, including wav2vec 2.0 features \cite{baevski2020wav2vec}, VQ-APC features \cite{chung2020vector}, our previously proposed DeCoAR features \cite{ling2020deep}, DeCoAR 2.0 features as proposed in this work. For wav2vec 2.0 features \cite{schneider2019wav2vec}, we obtained 768-dimensional representations from the wav2vec 2.0 base model downloaded from\footnote{https://github.com/pytorch/fairseq/tree/master/examples/wav2vec}, which was pre-trained on 960-hour LibriSpeech data with contrastive loss and had the exactly same encoding network as ours. For VQ-APC features, we trained a VQ-APC model using the official code\footnote{https://github.com/iamyuanchung/VQ-APC} provided by the authors on 960-hour LibriSpeech. We obtained 512-dimensional VP-APC representations as input features. DeCoAR and DeCoAR 2.0 have dimensionality of 2048 and 768, respectively. For all systems trained on learned speech representations, the downstream ASR model are 2 layers of bidirectional LSTMs with CTC loss. In line with our previous work \cite{ling2020deep}, we also train purely supervised systems using conventional filterbank features. These models are trained using 6 layers of bidirectional LSTMs with CTC loss. We also trained a purely supervised system using the entire 960-hour dataset uisng filterbank features as a baseline.


% Our experiments consisted of five different SSL system, trained on various acoustic representations including: 
% 1) Conventional filterbank features;
% 2) wav2vec 2.0 \cite{baevski2020wav2vec} features; 
% 3) VQ-APC \cite{chung2020vector} features; 
% 4) our previously proposed DeCoAR \cite{ling2020deep} features. 
% 5) DeCoAR 2.0 features as proposed in this work.


% We used \textit{dev-clean} for validation and \textit{test-clean}, \textit{test-other} for evaluation.  The output CTC labels were 71 phonemes\footnote{The CMU lexicon: \url{http://www.speech.cs.cmu.edu/cgi-bin/cmudict}} plus one blank symbol. All ASR task-specific models used were 2 BLSTM layers with the CTC loss criterion. 

% For comparison, we obtained 768-dimensional wav2vec 2.0 representations \cite{schneider2019wav2vec} from the wav2vec 2.0 base model\footnote{\url{https://github.com/pytorch/fairseq/tree/master/examples/wav2vec}}. Their model was pre-trained on 960-hour LibriSpeech data with constrastive loss and had the exactly same architecture as ours. And we also trained VQ-APC model using their official code\footnote{\url{https://github.com/iamyuanchung/VQ-APC}} on 960-hour LibriSpeech. We obtained 512-dimensional VP-APC representations for our ASR training data. We didn't look into fine-tuning option since models are trained in different toolkit and it won't be a fair comparison with different decoding setup.


% For evaluation purposes, we applied WFST-based decoding using EESEN \cite{miao2015eesen}. We composed the CTC labels, lexicons and language models (unpruned trigram LM for WSJ, 4-gram for LibriSpeech\footnote{Downloaded from \url{http://www.openslr.org/11}}) into a decoding graph. The acoustic model score was set to $0.8$ and $1.0$ for WSJ and LibriSpeech, respectively, and the blank symbol prior scale was set to $0.3$ for both tasks. We report the performance in word error rate (WER).

% \subsection{Semi-supervised LibriSpeech Results}
Table \ref{table:LibriSpeech} shows the results on semi-supervised LibriSpeech experiments. We conducted our semi-supervised experiments using 1 hour, 10 hours, and 100 hours of training data. Our proposed approach significantly outperforms the pure supervised filterbank baselines. In particular, under extremely data-sparse conditions, the proposed DeCoAR 2.0 methods achieved highly competitive performance, with a WER of 5.43\%/13.27\% for \textit{test-clean}/\textit{test-other} using 10 hours of labeled data, and a WER of 13.75\%/29.13\% for \textit{test-clean}/\textit{test-other} using only 1 hour of labeled data. One notable observation is that using 10 hours of labeled data can already outperform the system trained on the full 960-hour data with filterbank features by 6.7\%/8.5\% relative WER improvements on \textit{test-clean}/\textit{test-other}.  

Among different speech representations, wav2vec 2.0 and DeCoAR 2.0 performed favorably compared to VQ-APC and DeCoAR.  DeCoAR 2.0 is comparable to wav2vec 2.0 in all different SSL conditions as well. %In the 1-hour SSL condition, DeCoAR 2.0 has minor degregation over wav2vec 2.0. We further run an evaluation using greedy decoding without incorporating lexicon and LM information in WFST. The greedy decoding shows that the DeCoAR 2.0 achieved a phone error rate of 17.5\% on dev-clean, compared to 18.9\% with wav2vec 2.0. 
It is worth noting that we did not perform fine-tuning for all representation learning layers as these models were trained in different stacks. We are interested in gauging the performance comparison by directly using the resulting speech representations produced from different pre-trained speech representation models. 

%On the more challenging \textit{test-other} dataset, we also achieve performance on par with the filterbank baseline using a 360h subset. Furthermore, training with with our DeCoAR features approach improves the baseline even when using the exact same training data (960h). 

%Note that while \cite{park2019specaugment} introduced SpecAugment to significantly improve LibriSpeech performance via data augmentation, and \cite{luscher2019rwth} achieved state-of-the-art results using both hybrid and end-to-end models, our approach focuses on the SSL case with less labeled training data via our DeCoAR features.


% \subsection{Ablation Study and Analysis}

% \subsubsection{Without VQ layer}
We conduct an ablation study to investigate the effect of inserting VQ layer in DeCoAR 2.0 in Table~\ref{table:vq_layer}, and confirm the VQ module is beneficial for ASR tasks. We hypothesize that vector quantization forces the DeCoAR model to reduce the model capacity and focus more on informative factors such as linguistic/phonetic unit discovery and less so on other factors such as speaker traits, acoustic condition. 

% reconstruction task utilizes all the information available (speaker traits, background noise, etc.) to achieved maximal prediction while those information are less relevant to ASR. With the addition of a VQ layer, these unwanted information are limited into final representation. .

\begin{table}[thb]
    \centering
    \ninept
    \begin{tabular}{ c | cc  }
        \toprule
        {\textbf{VQ}} & {\textbf{test clean} } & {\textbf{test other} } \\
        \midrule
        \xmark &  6.29 & 18.54 \\
        %15 & & \\
        \cmark & 5.43  & 13.27\\
        \bottomrule
    \end{tabular}
    \caption{Ablation on the effect of using VQ layer on the Librispeech 10 hours SSL experiment.}
    \label{table:vq_layer}
\end{table}



==> decoar 2.0/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we present vector quantized \textbf{De}ep \textbf{Co}ntextualized \textbf{A}coustic \textbf{R}epresentation (DeCoAR 2.0), an improved speech representation learning approach based on DeCoAR and vector quantization.  DeCoAR 2.0 has multiple modification over the its predecessor, with a deep Transformer as encoding block, and the addition of a vector quantization module before reconstruction module. In extreme data-limited semi-supervised conditions, we observe that using 10 hours of labeled data with DeCoAR 2.0 achieved performance on par with the system trained on 960 hours of conventional filterbank features. DeCoAR 2.0 also performed comparably to wav2vec 2.0 in all different semi-supervised scenarios. Future work includes exploring the efficacy of representation learning in real world data including noisy and adverse conditions, and extension to neural transducers \cite{rao2017exploring,li2019improving} and other end-to-end ASR systems as downstream tasks. 

% In this paper, we introduce a novel self-supervised representation learning approach. We first propose a novel objective for a deep transformer network, where large amounts of unlabeled data are used to learn vector quantized deep contextualized acoustic representations (DeCoAR 2.0). These DeCoAR 2.0 features are used as the representations of labeled data to train a CTC-based end-to-end ASR model. In our experiments, we achieve similar performance to training on 960 hours of labeled by pretraining then using only 10 hours of labeled data. 

